Accelerating Deep Learning Inference via Learned Caches

Deep Neural Networks (DNNs) are witnessing increased adoption in multiple domains owing to their high accuracy in solving real-world problems. However, this high accuracy has been achieved by building deeper networks, posing a fundamental challenge to the low latency inference desired by user-facing applications. Current low latency solutions trade-off on accuracy or fail to exploit the inherent temporal locality in prediction serving workloads. We observe that caching hidden layer outputs of the DNN can introduce a form of late-binding where inference requests only consume the amount of computation needed. This enables a mechanism for achieving low latencies, coupled with an ability to exploit temporal locality. However, traditional caching approaches incur high memory overheads and lookup latencies, leading us to design learned caches - caches that consist of simple ML models that are continuously updated. We present the design of GATI, an end-to-end prediction serving system that incorporates learned caches for low-latency DNN inference. Results show that GATI can reduce inference latency by up to 7.69X on realistic workloads.

==> sections/background_and_motivation.tex <==
\section{Background and Motivation}

We begin by providing a primer on Deep Learning and prediction serving of Deep Neural Networks (DNNs)(Section~\ref{subsec:dl_background}).
We discuss the goals of prediction serving and why current solutions fall short on achieving these goals (Section~\ref{subsec:pred_serving}).
We then outline how caches can speed up DNN prediction serving and discuss why {\em traditional caching} approaches are insufficient (Section~\ref{subsec:caching_background}).
This motivates the need for a new {\em learned caching} approach.

\subsection{Deep Learning Background}
\label{subsec:dl_background}
A Deep Neural Network (DNN) consists of a sequence of layers, each of which is responsible for applying a mathematical function on the output of the previous layer. These functions may be transformations (fully connected layers, pooling layers, convolutional layers, etc) or activation functions (ReLU, sigmoid, softmax, etc). We refer to the first layer of the DNN that accepts the input sample as the {\em input layer} and the final layer of the DNN that represents the final prediction as the {\em output layer}. We term the remaining intermediate layers of the DNN as {\em hidden layers}.

The Deep Learning lifecycle consists of two phases - training and inference.
Training involves learning a model that best fits the input dataset.
This entails learning weights associated with each layer of the DNN using algorithms like Stochastic Gradient Descent (SGD), that repeatedly iterate over the dataset until convergence.
During the inference or prediction phase, the trained model is deployed to serve applications.
Inference involves taking in an input sample and performing a forward pass in order to arrive at a prediction at the output layer.
In this work, we focus solely on the prediction serving phase and analyze the goals and challenges below.

\subsection{Prediction Serving}
\label{subsec:pred_serving}
\noindent{\bf Prediction Serving Goals. }

\noindent{\bf (G1) Low Latency } Prediction serving or inference requires {\em low latency} because the trained models are typically deployed to serve user-facing applications.
Emerging applications like interactive video analytics, voice assistants, and autonomous systems require quick responsiveness.
\todo{Shivaram: Can we use an example from the DeepCPU talk which has actual latency targets for
webapps? The autonomous driving application is way more complex and it has a lot of assumptions}
For instance, consider the example of autonomous driving vehicles.
One component of such a system would be an image recognition module that is responsible
for detecting traffic signs.
The module would receive a series of images from a video camera as input
and would be responsible for detecting the presence of traffic signs if any.
To react quickly to the presence of traffic signs, the module would need to be highly responsive and serve requests
with low latency. Modern-day image recognition utilizes deep learning~\cite{} and hence
low latency becomes a fundamental requirement when DNNs are used in such applications.



\noindent{\bf (G2) High Accuracy } \todo{keep these
explanations short?} The success of deep learning has led to its adoption in critical applications like finance and
domains that implicate human safety such as fraud detection and autonomous systems.
In such domains, errors can be costly and have huge negative impacts.
Consider the same example of an image recognition module within an autonomous driving system.
A mis-prediction regarding the presence or the type of a traffic sign could
potentially lead to fatal accidents.
With DNNs being used in such applications, high accuracy of predictions becomes a fundamental requirement.
\todo{Again these examples are less convincing without actual numbers in them. Instead say something
like ppl spend ages parameter tuning to get a few percent better accuracy? Again give concrete
numbers from even say a blog post or news article or papers on parameter tuning}

\noindent{\bf Challenges in Prediction Serving. }
Today, DNNs have surpassed human-level accuracy in tasks like 
image classification~\cite{}, speech recognition~\cite{}, and machine translation~\cite{}.
Consequently, prediction serving systems based on DNNs can offer high accuracy.
However, this high accuracy has been achieved by employing deep models with a large number of layers.
This poses a fundamental challenge to the goal of low latency since deeper models lead to inflated prediction latencies.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/Convolution_computation_node.pdf}
	\caption{Computation dependency between two successive layers of a DNN}
	\label{fig:dnn-computation-structure}
\end{figure}

To motivate why low latency is a fundamental challenge in deeper DNNs,
let us consider a canonical example (Figure~\ref{fig:dnn-computation-structure}) which consists of a convolution layer followed by a layer that applies ReLU activation.
\footnote{Note that this is not representative of any particular DNN architecture and the arguments we make can be generalized to any DNN architecture.}
We observe that the computation of the convolution layer can be parallelized
since the convolutional filter can make a pass over the input in parallel.
In modern accelerators such as GPUs that inherently support highly parallel workloads, this operation can be performed efficiently and does not lead to an inflation in latency.
While proceeding with the computation of the ReLU layer however,
one immediate observation we can make is that the computation of the ReLU layer only proceeds once the results of computation from the convolution layer are available.
This dependency between computations of successive layers can be captured using a Directed Acyclic Graph (DAG)
as shown in Figure~\ref{fig:dnn-computation-structure}, where each node represents a sub-computation within each layer of the DNN
and the arrows represents the dependencies between these sub-computations.
The latency of a prediction request depends on two properties of this DAG -
(i) The latency induced by individual nodes in the DAG.
(ii) The length of the critical path of the DAG.
With models becoming deeper, the length of the critical path of the DAG increases, leading to inflated prediction latencies.
%Thus, the highest achievable parallelism in prediction serving is a form of {\em pipelined parallelism}, where a portion of the ReLU computation can begin once the result of a task is available. Hence, while the computation every layer can be parallelized efficiently, parallelism across layers is limited by {\em pipelined parallelism}. Thus, the latency of a DNN prediction is dictated by the {\em length of the pipeline}, that is, the number of layers in the DNN. Deeper neural networks with a large number of layers thus pose a fundamental challenge to achieving {\em low latency}.

\noindent{\bf Current solutions. }
There are a myriad of solutions that use both algorithmic and systems techniques to reduce prediction latency.
We can categorize the prior solutions based on how they manipulate the computation DAG as below -

\noindent{\bf (C1) Reducing cost of individual nodes. }
One potential way to reduce prediction latency would be to reduce the cost of individual nodes of the DAG,
which cumulatively leads to a reduction in prediction latency.
The {\em quantization} of model weights~\cite{} is a popular technique
that reduces the cost of individual nodes in the DAG by reducing the
{\em precision} of computation.

\todo{Talk about pruning as well here.}

\noindent{\bf (C2) Reducing length of critical path. }
Other approaches typically reduce prediction latency by reducing the length of the critical path of the DAG,
usually by reducing the number of layers in the network.
The ResNet family of models used for image recognition tasks has an array of variants
(ResNet-18, ResNet-34, ResNet-50, ResNet-152, and so on),
each of which has different number of layers.
An application can pick a variant depending upon the latency requirement
and can thereby control the length of the critical path of the DAG.
{\em Distilling the knowledge} of a deep neural network into a smaller network is
another popular technique that can reduce the critical path length.


\noindent{\bf (C3) Utilizing multiple DAGs with different critical path lengths. }
Another approach to bound the prediction latency would be to consider an array
of DAGs and allow an application to choose one or more of these DAGs to serve
the prediction.
An application can make this choice depending upon factors such as the available
latency budget or the type of input.
{\em Ensemble} methods employed in systems such as Clipper~\cite{}
provide multiple models that perform the same task and use application-level
inputs such as latency budget to determine which model to use during the inference runtime.
Other systems such as NoScope~\cite{} provide {\em specialized models}
that forego generality and 
offer low latency for common queries in video analytics settings.
These specialized models are used in conjection with generic models, resulting
in a {\em cascade} of model being used for prediction serving.

\noindent{\bf Limitations of current solutions. }

\todo{Add figure for latency-accuracy trade-off space. Shivaram: Actually put it in the introduction}

\noindent{\bf (L1) Workload-unaware with fixed, early binding on the latency-accuracy trade-off. } 
A myriad of DNN architectures are available for performing the same task.
Coupled with techniques that reduce the computational cost of a node in the DAG or reduce the
length of the critical path in the DAG, these represent a rich space of solutions that provide
different accuracy and latency properties.
Figure~\ref{} shows that accuracy and latency typically trade-off
and that current solutions occupy a {\em fixed} point in this trade-off space.
By committing to a particular DNN architecture or technique to reduce DAG computational costs
prior to prediction serving,
we observe that current solutions inherently {\em early-bind} to a particular point in the
trade-off space. \todo{again too many emphs} \aditya{the rest of the sentences seem repetitive. Also, an issue is that this para does not say what the problem with workload awareness or early-binding is! it merely observes that unawareness and early-binding exist today. need to say what tangible ideal benefits can arise from dynamic binding and workload awareness}
Thus, current solutions offer static properties of latency and accuracy
and leave no room for dynamically manipulating these properties
based on the prediction serving workload. Thus, existing techniques optimize for
latency in a workload unaware manner.

\todo{Emperical evidence that workload awareness helps?}

\noindent{\bf (L2) Modify DNN architecture. }
Some of the current solutions reduce prediction latency either by modifying the original structure of the DNN (e.g. distillation)
or by using multiple variants (e.g. Clipper~\cite{}, NoScope~\cite{}).
In such techniques, the model typically needs to be trained with the modified architecture(s).
Training specialized models to be deployed for predcition serving typically takes a lot of time~\cite{}
and requires large amounts of expensive resources such as GPUs.
Additionally, such techniques might impact the fidelity of predictions.
It is well known that a considerable amount of resources get used up in identifying the right model architecture for a given task (e.g. hyperparameter exploration).
Training specialized models for prediction serving would require this level of fine tuning
to be carried out again and is therefore a costly affair in practice.
\todo{why not say that ensemble requires more resources?}

\aditya{not sure I understand the point of L2. I don't see a separate noteworthy point there. Aren't these modified archs also picking a specific point in the trade-off space. Aren't they also workload unaware? I suggest combinining L1 and L2 and just listing out a bunch of issues.}
   
\subsection{Exploring the accuracy-latency trade-off space}
\label{subsec:caching_background}

Given that current approaches suffer from key limitations,
we need to explore new techniques to speed up prediction serving
that avoid such a static binding and do not involve
modifying the original DNN architecture.


\noindent{\bf A caching proposal. }
%Given that current approaches suffer from key {\em limitations}, we need to explore new techniques to speed up prediction serving
Over the years, caching has helped speed up several applications~\cite{}.
We believe that the prediction serving workload is naturally amenable to caching.
It is a well known fact that online workloads typically follow a Zipfian distribution~\cite{zipf}.
Additionally, workloads such as video analytics have almost similar input frames across time
and thus we believe that \emph{caching} DNN computations can speed up prediction serving.


\begin{figure}[t]
  \centering
   \includegraphics[width=0.4\textwidth]{figures/Intuition_Combined.png}
    \caption{A basic caching mechanism where (a) The hidden layer outputs along with the associated predictions are cached.
	(b) During inference, a cache look-up is done after every layer and a cache hit yields a faster prediction}
    \label{fig:traditional_caching}
\end{figure}

Figure~\ref{fig:traditional_caching} illustrates a simple mechanism to realize the caching of DNN computations.
As a pre-processing step, from the validation dataset, we can cache the hidden layer outputs along with the final predictions delivered by the DNN.
During prediction serving, we lookup the cached hidden layer outputs.
If a hidden layer output matches what was cached earlier, we deem this as a {\em cache hit}
and can skip performing computations for the remaining layers and directly deliver the final prediction.

Caching of DNN computations helps overcome the
limitations of current solutions that we outlined earlier.
As illustrated in Figure~\ref{fig:traditional_caching}, with caching, prediction requests will now have a wide range of
latencies depending on which hidden layer of the DNN yields a cache hit.
With this, caching paves the way for {\em late-binding} onto a point in the accuracy-latency trade-off
space. 
Caching opens up an entire {\em latency spectrum} that is dependent on the properties of the prediction request. \aditya{what is the resulting benefit? what you have listed here is just an observation.}
Additionally, a cache simply supplements a DNN and does not require modifying the DNN architecture.
Thus, caching is a promising technique that can be exploited.
%Caching can overcome the bottleneck imposed by pipelined parallelism by {\em reducing the effective length of the pipeline}.
%Thus, caching of DNN computations is a promising approach to reduce prediction serving latency.

\noindent{\bf Issues with traditional caching approaches.} \aditya{instead of issues with traditional approaches, I suggest writing this as challenges in realizing cachibe. the main issue is that there are no ``traditional'' approaches to consider here. i would figure out how to write the challenges so as to motivate the need for a learned cache approach.}
While caching offers hope, there exist several issues that render a traditional caching approach like we described above ineffective.
Most issues stem from the fact that the hidden layer outputs typically reside in {\em high dimensional} space.
We highlight the issues below -

\noindent {\bf Memory Overheads. }
High dimensionality inflates the amount of memory required to store
cached computations. This memory overhead becomes a major problem
in accelerating co-processors such as GPUs which have limited DRAM capacity (typically 16-32GB). \aditya{this is too vague - give precise numbers}
This severely restricts the amount of computations that can be cached and thereby the efficacy of caching.

\noindent {\bf Fidelity of cache lookup. }
High dimensionality also means that a cache lookup based on {\em exact matches} are unlikely~\cite{}.
Thus, a cache lookup would instead involve looking for the closest available cached prediction.
However, this presents an issue since distance-based similarity metrics
do not work with high fidelity in high dimension~\cite{}. \aditya{I don't like talking about a fake caching scheme, and then poking holes at it. This point about fidelity can be argued as - we can't use traditional cache design approaches such as exact hits or nearby hits (similar to LSH)}

\noindent {\bf Inflated lookup latencies. }
Due to the need to perform distance computations to find the closest available cached prediction,
high dimensionality also inflates the latency associated with a cache lookup
and renders cache lookup extremely expensive.
Additionally, the cost increases with an increase in the number of cached data points . \aditya{drop this? this seems very specific to a particular broken strawman cache design}

All of the above
mentioned issues motivate the need for developing improved % {\em impro}
caching mechanisms for DNN prediction serving. \aditya{rewrite this lead out if you are going to re-pitch the above issues as challenges in caching}

%\arjun{Is the above strong enough or do we need to support the arguments with numbers?}
\todo{Having some numbers is always good. Especially for the latency of cache lookup thing try to
add some?}


==> sections/evaluation.tex <==
\section{Evaluation}

We evaluate \name{} to answer the following questions:

\begin{itemize}

	\item How advantageous is late-binding in \name{} over early-binding techniques?
		Does it meet our goal of reducing prediction serving latency while retaining high accuracy?
		How do various design choices adopted in \name{} help in achieving this goal?
	\item How much benefit does query replanning offer in increasing the end-to-end accuracy for multi-DNN queries?
	\item How well does \name{} adapt to temporal locality in the input request distribution? What are the
	      parameters in the cache updation service that impact the effectiveness of this adaptation?
\end{itemize}

\noindent {\bf Experimental Setup: }
We evaluate a prototype implementation of \name{}
deployed on a heterogeneous cluster
comprising of 10 p3.2xlarge GPU instances~\cite{awsec2}
and 4 t3.xlarge CPU instances~\cite{} on AWS.
Each GPU instance has 1 NVIDIA Tesla V100 GPU and 18 CPU cores.
We run the daemons for the query scheduler, initial model
upload, inference service, and cache updation service on
dedicated CPU instances.
In our evaluation, we allocate 8 GPU instances for learned
cache construction.
Since, learned cache construction is a one-time operation,
we use the same 8 GPUs to constitute the cache updation service.
Our inference service consists of 2 GPU instances.
\todo{Need to clearly outline here that this is reasonable scale.
We run only one workload at a time and this cluster size suffices.
There is no fundamental reason for Freeze to not scale.}
Each DNN model along with the associated learned caches
resides on its own dedicated GPU instance.
For CPU inference, we use the same GPU instance and constrain
the computation to run on the CPU.
We allocate 8 CPU cores for the base model computation and 8
CPU cores for the learned cache computation.

\noindent {\bf Default Parameters: }
We consider three predictor network architectures -
fully-connected, pooling, and convolution along
with two hyper-parameters for each architecture.
This results in six different learned cache variants
being considered - FC\_Arch(H=1024), FC\_Arch(H=512),
Pool\_Arch(H=8192), Pool\_Arch(H=4096),
Conv\_Arch(K=3,S=1), Conv\_Arch(K=5,S=2) (same as in Table~\ref{tab:exploration_tradeoff}).
We tune the value of $\delta$ in the selector networks so as to achieve an
accuracy of greater than 97\%.
In the composition phase, we choose the accuracy target A to be 97\%.
Across all experiments, we choose the memory budget to be 10 GB, which 
is the minimum available memory budget across all deployments.
This budget is sufficiently large enough to hold the most optimal set of learned caches.
We evaluate the performance of \name{} under memory pressure in \secref{}.
We assume that at most one learned cache lookup can be computed at
given point of time.

\noindent {\bf Target Hardware: }
Inference services are run both on CPUs~\cite{}
as well as on accelerators such as GPUs.
We consider both these hardware in our evaluation.

\subsection{Late binding benefits}

In this section, we evaluate the benefits of late-binding the amount
of computation to be performed.
To focus on this aspect, we deploy \name{} with the
cache updation service disabled, so that the inference
service uses only the initial constructed set of learned caches.

\noindent {\bf Datasets and Workload: }
We use four model-dataset pairs
to evaluate the benefits of late binding in \name{}.
Our evaluation considers popular image classification
(CIFAR-10 and CIFAR-100~\cite{cifar}) and speech recognition
(Google Commands~\cite{}).
We also consider 4 different base DNN architectures: VGG-16~\cite{}, ResNet-18,
ResNet-50, ResNet-152~\cite{}. These represent state-of-the-art DNNs
that have a different number of layers.

We use the training data from each dataset to train the predictor and selector
networks for all learned cache variants.
In our setup, the initial cache construction uses 80\% of the training data,
sampled at random
for training each predictor/selector network. The remaining 20\% is used as validation
dataset for the selector network and used for obtaining the
hit rate and accuracy for use in the composition phase.
The test set of the dataset is fed to the inference service at a constant
rate so as to prevent any queuing at the scheduler\footnote{
We do not evaluate \name{} with batching, but discuss its implications in \secref{}}.

\noindent {\bf Baselines: }
We evaluate the benefits of late binding by comparing \name{}
to different early binding techniques as outlined in
\secref{subsubsec:current_solutions} -
(i) Quantization~\cite{}, where the base DNN is quantized to yield models
that use a varying number of bit-widths.
(ii) Model distillation~\cite{}, where the base DNN is distilled into
student models having a varying number of layers
(iii) Model pruning via Network Slimming~\cite{}, where the
base DNN is pruned by varying percentage levels.
Additionally, we also compare \name{} to computing the entire
base DNN.

\noindent {\bf Metrics: }
Since each baseline technqiue occupies a different
region in the latency-accuracy trade-off space as shown in Figure~\ref{},
we compare \name{} separately with each baseline technique.
We use metrics along two dimensions for our comparison as outlined below -
(i) The spectrum of latencies offered by
\name{} against the latency offered by the baseline technique.
We use the observed average latency using \name{} as a single
point of comparison against the baseline technique.
inference.
(ii) We compare the accuracy of prediction offered
by \name{} and baseline techniques. Crucially, we define
accuracy to be the percentage of inference requests
for which the output matches the prediction of the base DNN.
This measures the ability of the technique to mimic the
behavior of the base DNN, a desirable property when
construct low latency derivatives from the base DNN.

\subsubsection{Results}

\begin{comment}




\begin{figure}[t!]
        %\centering
        \subfloat[][Latency comparison]{\includegraphics[width=0.49\columnwidth]{figures/res152-macro-cpu-latencies.pdf}}
        \subfloat[][Latency vs. accuracy]{\includegraphics[width=0.49\columnwidth]{figures/res152-macro-cpu-accuracies.pdf}}
        \caption{\label{fig:res152-macro-results-cpu} [CPU inference] Benefits of late-binding for 
        ResNet-152 on CIFAR-100 dataset. In (b),
        each dot for \name{} is sized in proportion to the number of inference requests
        served at that particular latency point.}
\end{figure}

\begin{figure}[t!]
        %\centering
        \subfloat[][Latency comparison]{\includegraphics[width=0.49\columnwidth]{figures/res152-macro-cpu-latencies.pdf}}
        \subfloat[][Latency vs. accuracy]{\includegraphics[width=0.49\columnwidth]{figures/res152-macro-cpu-accuracies.pdf}}
        \caption{\label{fig:res152-macro-results-cpu} [CPU inference] Benefits of late-binding for
        ResNet-152 on CIFAR-100 dataset. In (b),
        each dot for \name{} is sized in proportion to the number of inference requests
        served at that particular latency point.}
\end{figure}




\end{comment}

\begin{figure}[t!]
	%\centering
	\subfloat[][Latency comparison]{\includegraphics[width=0.49\columnwidth]{figures/res50-macro-cpu-latencies.pdf}}
	\subfloat[][Latency vs. accuracy]{\includegraphics[width=0.49\columnwidth]{figures/res50-macro-cpu-accuracies.pdf}}
	\caption{\label{fig:res50-macro-results-cpu} [CPU inference] Benefits of late-binding for 
	ResNet-50 on CIFAR-10 dataset. In (b),
	each dot for \name{} is sized in proportion to the number of inference requests 
	served at that particular latency point.}
\end{figure}
\begin{figure}[t!]
        %\centering
        \subfloat[][Latency comparison]{\includegraphics[width=0.49\columnwidth]{figures/res50-macro-gpu-latencies.pdf}}
        \subfloat[][Latency vs. accuracy]{\includegraphics[width=0.49\columnwidth]{figures/res50-macro-gpu-accuracies.pdf}}
        \caption{\label{fig:res50-macro-results-gpu} [GPU inference] Benefits of late-binding for 
        ResNet-50 on CIFAR-10 dataset. In (b),
        each dot for \name{} is sized in proportion to the number of inference requests 
        served at that particular latency point.}
\end{figure}
\noindent {\bf CIFAR-10 on ResNet-50: }
Figure~\ref{fig:res50-macro-results-cpu}(a) shows the distribution of latencies
of inference requests for \name{} against the baselines on CPU.
\name{} exhibits an average latency of \textasciitilde {\bf 34 ms}, which is
{\bf 1.95$X$} lower than the latency of running the entire DNN.
Figure~\ref{fig:res50-macro-results-cpu}(b) shows that \name{} exhibits
a spectrum of latencies with an overall accuracy of {\bf 96.97\%} with respect
to the base ResNet-50 model, which is very close to the accuracy target of 97\%.
\name{} outperforms both 8-bit and 10-bit quantization by improving average latencies by a factor
of 1.74$X$ and 1.25$X$ respectively while also improving accuracy by 0.57\% and 0.97\% respectively.
With respect to 12-bit quantization, \name{}'s accuracy is \textasciitilde1\% lower but it provides
a more competitive latency profile with {\bf \textasciitilde76\%} of points having lower latency.
\name{} outperforms ResNet-50 distilled to ResNet-34 with an average latency improvement of 1.41$X$
and an accuracy improvement of 0.57\%. ResNet-50 distilled to ResNet-18 and a simple 5-layer CNN
have better average latency than \name{} but have accuracies lesser by {\bf 3.39\%} and {\bf 11.21\%} respectively.
\name{} has better accuracies than pruning at 50\%, 60\%, and 70\% while the average latency is only
1.02$X$-1.04$X$ worse-off. \name{} has comparable accuracy and average latency to pruning at 40\%,
but offers better latency for {\bf 73.85\%} of the requests.

Similarly, Figure~\ref{fig:res50-macro-results-gpu}(a) shows that \name{} exhibits an
average latency of \textasciitilde {\bf 7.98 ms}, which is {\bf 1.63$X$} lower than running ResNet-50 on a GPU.
Figure~\ref{fig:res50-macro-results-gpu}(b) shows that \name{} exhibits
a spectrum of latencies with an overall accuracy of {\bf 96.8\%} with respect
to the base ResNet-50 model. Once again, this aligns very closely with the accuracy target of 97\%.
\name{} outperforms quantization in terms of average latency by a factor of 1.08$X$(6-bit)-1.27$X$(12-bit).
Except for 12-bit, \name{} also offers better accuracy than the quantization baselines.
\name{} outperforms ResNet-50 distilled to ResNet-34 with an average latency improvement of 1.07$X$
and an accuracy improvement of 0.7\%. ResNet-50 distilled to ResNet-18 and a simple 5-layer CNN
have significantly lower average latencies but have accuracies lesser by {\bf 3.53\%} and {\bf 11.34\%}
respectively.
\name{} has better accuracies than pruning at 50\%, 60\%, and 70\%, while also improving average
latency by a factor of {\bf 1.39$X$-1.42$X$}. Pruning at 40\% has higher accuracy, but
\name{} offers better latency for {\bf 70.36\%} of the requests.

\noindent{\bf Other models and datasets:}
To further compare \name{} against early-binding techniques,
we evaluate \name{} on three more model-dataset pairs.
We observe similar trends as CIFAR-10 on ResNet-50 and
outline only the key highlights below -


\todo{Add more conclusions.}
\subsubsection{Sources of Improvement}

We now analyze the impact of specific design choices adopted by \name{}
that enable better latencies while ensuring that the accuracy is
close to the target accuracy.

\noindent {\bf Using learned caches: }
\begin{footnotesize}
\begin{table}[t]
  \centering
  \begin{tabular}{ l | c | c | c | c }
    \hline
	  \textbf{Scheme} & \shortstack {\bf GPU \\ \bf Lookup \\ \bf Latency \\ \bf (ms)  } & \shortstack {\bf CPU\\ \bf Lookup \\ \bf Latency \\ \bf (ms)  } & \shortstack{ \bf Memory\\ \bf(MB)} & \textbf{Accuracy} \\
    \hline
	  \textbf{k-NN (k=50)} & 2075.5 & & 5000 & 79.84 \% \\
    \hline
	  \textbf{LSH} & 71.4 & & 5000 & 39.77\% \\
    \hline
	  \shortstack{ \bf k-means \\ \bf (k=100)} &1.511 & & 333 & 76.06\% \\
    \hline
	 \shortstack {\bf Learned \\ \bf Cache \\ \bf (Conv\_Arch: \\ \bf K=3,S=1) }  & 0.48 & & 39 & \\
    \hline
  \end{tabular}
        \caption{Comparing learned cache against alternative caching approaches}
  \label{tab:trad_vs_learned}
\end{table}
\end{footnotesize}

Learned cache outperforms traditional cache in terms of cache hit rate. We construct traditional caches by storing the intermediate layers of the DNN with predictions in cache and performing either Locality Sensitive Hashing or k-nearest neighbors search to do approximate cache look-up. We construct k clusters out of the intermediate layers and store the majority label of each cluster in the k-means approach. Figure~\ref{fig:learned_cache_res18} shows that learned cache matches the cache hit rate of Locality Sensitive Hashing and k-nearest neighbors approaches up to block 4 while learned cache surpasses the two approaches by 2$X$ at block 5 and 2.4$X$ and 2.67$X$ for KNN and Locality Sensitive Hashing respectively. Learned cache matches the cache hit rate of k-means clustering up to block 3. Although k-means clustering outperforms learned cache for deep blocks, it comes at the cost of reduced accuracy from 96.67\% of learned cache to 92.85\%.

\begin{figure}[t!]
        %\centering
        \subfloat[][Using distillation loss function in predictor network]{\includegraphics[width=0.49\columnwidth]{figures/distillation_loss_res50_gpu.pdf}}
        \subfloat[][Decoupling prediction and selection into separate networks]{\includegraphics[width=0.49\columnwidth]{figures/selector_res50_cpu.pdf}}
        \caption{\label{fig:distillation_loss_res50_gpu} (a) [GPU Inference]Comparison between distillation loss function and cross entropy loss function in predictor networks for ResNet-50 on CIFAR-10 dataset, (b) [CPU Inference]comparison of using selector networks and setting thresholds to predictor networks for ResNet-50 on CIFAR-10 dataset}
\end{figure} 

\noindent {\bf Using distillation loss function in predictor network: }
We outlined in Section~\ref{sec:learned_cache} that we use a loss function that
borrows from knowledge distillation~\cite{} instead of a standard cross-entropy loss function
for training the predictor network.
Figure~\ref{fig:distillation_loss_res50_gpu}(a) shows that using the distillation loss 
gives a greater number of cache hits at earlier layers.
As an example, 34.77\% of requests have a latency of less than 5 ms using the distillation loss function,
while this is 3.47\% for the cross-entropy loss function.
This improvement stems from the fact that using the distillation loss function
results in more accurate predictor networks, thereby allowing the selector network
to infer more points as confident cache hits.
Overall, we observe a {\bf 5.9\%} improvement in accuracy by using the distillation loss function.

\noindent {\bf Decoupling prediction and selection in learned caches: }
We outlined in Section~\ref{sec:learned_cache} that we use learned caches employ two separate
networks for cache prediction and infering a cache hit.
Decoupling the decisions helps give cache hits with the desired
accuracy and hit rate properties.
We compare this choice against a baseline that uses only the
predictor network and establishes a threshold over the softmax scores
from the predictor network to infer cache hits.
We notice from Figure~\ref{fig:distillation_loss_res50_gpu}(b) that applying
different thresholds on predictor networks
induces trade-offs between accuracy and hit rate that is hard to control.
The selector network provides a binary classification mechanism
that allows for optimal control of the trade-off between accuracy and hit rate.
\begin{figure}[t!]
        %\centering
        \subfloat[][Exploring multiple predictor network architectures]{\includegraphics[width=0.49\columnwidth]{figures/model_variant_res50_cpu.pdf}}
        \subfloat[][Hardware aware profiling]{\includegraphics[width=0.49\columnwidth]{figures/hardware_aware_res50_cpu.pdf}}
        \caption{\label{fig:model_variant_res50_cpu} (a)[CPU Inference]predictor networks variants latency gain for ResNet-50 on CIFAR-10 dataset, 
        (b)[CPU Inference]hardware aware profiling vs hardware unaware profiling for ResNet-50 on CIFAR-10 dataset}
\end{figure} 

\noindent {\bf Exploring multiple predictor network architectures: } 
We saw in Section~\ref{subsec:exploration_phase} that \name{} explores multiple
predictor network architectures to get more visibility into the trade-off space
encompassed by the various learned cache metrics~\ref{tab:exploration_architectures}.
We evaluate the benefit of this design choice by comparing against exploration
phases that consider either only one type of network architecture
or only one hyper-parameter for each architecture.
While exploration does not impact the overall accuracy, we observe
from Figure~\ref{fig:model_variant_res50_cpu}(a), that exploring more
variants leads to better latency benefits, since it provides
more data points for the composition phase to pick from.
The minimum latency (5.57 ms) by considering all variants matches 
the minimum latency by considering only variants with pooling architecture.
Similarly, the median latency (27.5 ms) by considering all variants matches 
the minimum latency by considering only variants with fully-connected architecture.
Exploration thus gives combined benefits of exploring individual variants.
A trade-off incurred in exploring multiple variants is that it requires more
resources during the initial cache construction phase. Developers can limit
the number of variants to be explored depending upon the resource availability.

\begin{figure}[t!]
        %\centering
        \subfloat[][Alpha Regime CPU]{\includegraphics[width=0.49\columnwidth]{figures/alpha_regime_cpu.pdf}}
        \subfloat[][Memory Budgets]{\includegraphics[width=0.49\columnwidth]{figures/micro_memory_latency.pdf}}
        \caption{\label{fig:alpha_regime} $\alpha$ exploration during composition phase. (a) shows Latency/Accuracy tradeoff based on CPU profiling, 
        (b) [CPU Inference]Latency benefits offered by \name{} under reduced memory budgets}
\end{figure}
\noindent {\bf Optimal cache composition: }
The composition phase of \name{} uses a parameter $\alpha$ to
compute a score for each learned cache variant
and balance the inherent trade-off between latency gain and cache hit rate
(Equation~\ref{eqn:model_score}).
During the composition phase, \name{} evaluates multiple $\alpha$ values
and picks a value that minimizes the expected latency while maximizing accuracy.
For ResNet-50 on CIFAR-10, Figure~\ref{fig:alpha_regime}(a) shows that $\alpha$ 
values of 0.2 and 0.3 on CPU and GPU respectively provide optimal results.
\name{} selects the final set of learned cache variants based on these
$\alpha$ values.


Next, we illustrate the benefit of formulating the composition phase
as an optimization problem by comparing it to two greedy approaches -
(i) A latency greedy approach that greedily picks variants
with maximum latency gain while respecting computational and memory constraints.
(ii) A hit-rate greedy approach that greedily picks variants
with maximum hit-rate by respecting computational and memory constraints.
From Figure~\ref{fig:alpha_regime}(b), we observe that the optimization
problem has the most optimal latency profile, offering upto {\bf 5\%} improvement
in average latency.
This can be tied down to a better visibility
of the trade-offs between the various metrics for learned caches
that an optimization formulation can capture.

\noindent {\bf Hardware aware profiling: } 
In the composition phase, \name{} profiles the lookup latency
on the same target hardware where the model will be deployed for prediction serving.
Figure~\ref{fig:model_variant_res50_cpu}(b) shows that profiling in such a hardware-aware manner
offers latency benefits compared to having a composition phase that is hardware unaware.
We observe a {\bf 12.93\%} improvement in average latency and 
16.13\% of the requests have lower latency than the minimum latency (26.48 ms)
with hardware unaware profiling.


\noindent {\bf Asynchronous learned cache lookup: }
From Table~\ref{tab:exploration_tradeoff}, we observe that
lookup latencies can be comparable to computing a layer of the DNN.
Performing asynchronous cache lookups helps reduce tail latencies
and bounds the maximum latency from \name{} to the latency of running
the entire base DNN.
Across all of our macro-benchmark measurements, we note that
the tail latencies from \name{} are {\bf within 1\%} of the latency
of the base DNN.
We also observed that performing synchronous learned cache lookups can
inflate the tail latency by upto {\bf 50.11\%}.

\subsubsection{Overheads}
\todo{
	1. Memory overhead incurred.
	2. Extra hardware utilization incurred due to cache lookups.
	3. How long to explore, compose
}

\subsection{Query replanning benefits}

\todo{Need to include one cheaper model in each node to show more accuracy benefits}

\begin{figure}[t!]
        %\centering
         \includegraphics[width=0.8\columnwidth]{figures/query_replanning_workload.pdf}
        \caption{Structure of DNN query used for evaluating query replanning benefits}
        \label{fig:query_replanning_workload}
\end{figure}

\begin{footnotesize}
\begin{table}[t]
  \centering
  \begin{tabular}{ l | c | c | c }
    \hline
	  \textbf{Module} & \textbf{DNN} & \textbf{Latency} & \textbf{Accuracy} \\
    \hline
                               & ResNet-18 & 27.36 ms & 91.1\% \\
	  \textbf{Obj. Detect} & ResNet-34 & 41.05 ms & 92.9\% \\
	                       & ResNet-50 & 54.5 ms & 94.1\% \\
    \hline
	                       & SE-LResNet9E-IR & 17.38 ms & 95.5\% \\
			       & SE-LResNet18E-IR~\cite{} & 36.75 ms & 97.6\% \\
          \textbf{Face} & SE-LResNet50E-IR & 58.34 ms & 98.1\% \\
                               & SE-LResNet101E-IR & 110.32 ms & 99.1\% \\
    \hline
	                       & ResNet-9 & 16.14 ms & 90.2\% \\
	                       & ResNet-18 & 23.68 ms & 91.8\% \\
          \textbf{Vehicle} & ResNet-50 & 54.12 ms & 92.6\% \\
                               & ResNet-101 & 111.42 ms & 93.4\% \\
    \hline
  \end{tabular}
        \caption{List of DNNs models used in traffic analysis application}
  \label{tab:query_replanning_models}
\end{table}
\end{footnotesize}

In this section, we evaluate the benefits obtained by replanning the query execution
of upstream DNN executions
depending upon the latency observed from downstream DNN executions.
Once again, we deploy \name{} with the cache updation service disabled
so as to study the benefits of replanning in isolation.

\noindent {\bf Workload: }
We use a query DAG (Figure~\ref{fig:query_replanning_workload})
that resembles a traffic analysis application~\cite{}.
The input request first goes through an object detection module
that identifies if a face or vehicle is present in the input.
Depending on the outcome, the input is run through a vehicle
or face recognition module.
As shown in Table~\ref{tab:query_replanning_models}, we consider multiple DNNs 
for each module that have a varying number
of layers and consequently have different trade-offs in
latency and accuracy.
We use learned caches in the object detection module.
We sample images from the LFW dataset~\cite{},
Stanford Cars dataset~\cite{}, and CIFAR-100 and issue
them as input requests. The input distribution
used in this evaluation consists of 31\% faces and
27\% vehicles.
Each model is deployed on a separate instance
and uses CPU for inference.

\noindent {\bf Baselines: }
We consider both
the equal split and smart split policy as outlined in
\secref{subsubsec:query_planning}.
We evaluate the performance of \name{} with learned caches
and query replanning enabled in the query scheduler
against a vanilla baseline that does not use learned caches
or query replanning.
\begin{figure}[t!]
        %\centering
        \subfloat[][]{\includegraphics[width=0.49\columnwidth]{figures/equal_split_accuracy.pdf}}
        \subfloat[][]{\includegraphics[width=0.49\columnwidth]{figures/smart_split_accuracy.pdf}}
        \caption{\label{fig:replanning_equal_improvement} (a) Accuracy benefit obtained by query replanning in \name{} using equal split policy
        (b) }
\end{figure}

\begin{figure}[t!]
        %\centering
        \subfloat[][Sources of improvement]{\includegraphics[width=0.49\columnwidth]{figures/equal_split_sources.pdf}}
        \subfloat[][Latency profile]{\includegraphics[width=0.49\columnwidth]{figures/equal_split_sources_vehicle.pdf}}
        \caption{\label{fig:replanning_equal_sources} Insights into the benefits of query replanning using equal split policy}
\end{figure}


\noindent {\bf Result: }
From Figure~\ref{fig:replanning_equal_improvement}(a), we observe 
that query replanning with equal split policy gives
accuracy benefits for a variety of latency SLOs, offering upto to {\bf 0.984\%} improvement
in end-to-end accuracy.
Figure~\ref{fig:replanning_equal_sources}(a) provides insight into
why \name{} is able to give accuracy benefits.
At lower SLOs, we note that there is minimal accuracy benefit since fewer
requests get the opportunity to use more accurate models due to replanning.
The same effect is in play for higher SLOs, where both \name{} and the
baseline use the most accurate models for serving the queries.
The highest accuracy benefit comes in the middle range of SLOs where
we see that the additional latency slack obtained due to early
predictions from the object detection module can help
use more accurate models for face or vehicle detection.
We observe that this accuracy
improvement also comes with an improvement in the minimum and median latencies
for most latency SLO targets. At a latency SLO of 110 ms,
we observe that \name{} can reduce
average latencies by upto {\bf 1.16X} coupled with an accuracy improvement of {\bf 0.984\%}.
We observe similar trends for the smart split policy and omit the results here
for brevity.

\noindent {\bf Takeaway: }
Query replanning at the query scheduler helps reallocate additional slack to the
computed partial latency budgets. We observe that this enables models of higher
accuracies to be used for serving queries, thereby leading to greater end-to-end
accuracies. Crucially, this accuracy benefit also comes with improvements
in average latency.

\subsection{Cache Updation benefits}

4 video results here. E2E CDF in graph.
Accuracy in text

Pick some data from early block to show
why we get earlier cache hits.
Trend: Fine-tuning improves predictor accuracy,
which induces a greater percentage of cache hits
at earlier layers.

\subsubsection{Sensitivity Analysis}

\noindent {\bf Impact of class distribution in workload: }
Show Zipfian 1.5 vs Zipfian 3 latency CDF.
We expect more benefits with more skewed distributions.

\noindent {\bf Update interval: }
Show timeline graph zoomed in.
There is sensitivity to update interval.
Missing an update can miss out on opportunities to
exploit temporal locality. Operator needs to tune
this knob carefully according to workload.

\noindent {\bf Impact of sampling: }
Show E2E CDF with different sampling percentages on a macro-benchmark video.
Minimal sampling can still give good benefits.

\subsubsection{Overheads}

\subsection{Micro-benchmarks}

\noindent {\bf Memory budget: }
In the macro-benchmarks, \name{} had enough memory budget in both
the CPU and GPU inference to accommodate all learned caches
without memory being a bottleneck.
In this experiment, we evaluate the performance of \name{} under
reduced memory budgets. We emulate this in our testbed by
giving reduced memory budgets in the composition phase.


From Figure~\ref{fig:alpha_regime}(b), we notice that the latency
benefits offered by \name{} diminshes with a reduction in the
memory budget. When memory is not a bottleneck (10 GB), \name{}
improves average latency by 1.62$X$ with respect to the base model.
Under a reduced memory budget of 1 GB, the average latency degrades
only by a factor of {\bf 1.13X} and is still {\bf 1.44X} better than
the base model.

Additionally, we note that \name{} responds to reduction in
memory budget by choosing learned cache variants that have
smaller memory footprints. With a budget of 10 GB, we notice
that 6 of the 13 chosen variants have a fully-connected
architecture, which has a greater memory requirement.
With a budget of 1 GB, \name{} chooses only variants
with pool and convolutional architectures, which have a
smaller memory footprint.

\noindent {\bf Impact of accuracy target: }
\todo{Show that for tighter accuracy targets, we still get latency benefits.}

\noindent {\bf Query replanning on deeper query DAGs: }
\todo{Show accuracy benefit delta as depth of DAG varies.}


==> sections/key-ideas.tex <==
\section{Towards learned caches}

\begin{figure}[t]
        \centering
        \includegraphics[width=0.8\columnwidth]{figures/traditional_cache_vs_learned_cache.pdf}
        \caption{Difference between traditional and learned cache}
        \label{fig:traditional_vs_learned}
\end{figure}

To address the challenges mentioned in the previous section,
we propose adopting a learning-based approach for caching.
Instead of complementing each layer of the DNN with a traditional cache consisting of data,
our key idea is to use a machine learning model to represent the cache as shown in Figure~\ref{fig:traditional_vs_learned}.
We train a model that mimics a cache lookup function and term this as a {\em learned cache}.
The interface exposed by a learned cache remains the same as a traditional cache; i.e.,
the learned cache takes in a hidden layer output and delivers a prediction in the event of a cache hit.

Using a learned cache alleviates the issue associated with high dimensionality.
ML models are effective at handling high dimension input features~\cite{},
thereby allaying concerns about the fidelity of cache lookups.
A learned cache does not actually store any data 
but is instead a succinct cache representation encapsulated by the weights of the model.
Interestingly, the size of a learned cache 
depends on the model architecture and is independent of the number of items that constitute the cache.
Thus, we get a useful property that a learned cache can be used to encapsulate
a large number of cached predictions without having any implications on the memory requirement.
Third, the latency of a learned cache lookup is dictated by the cost
of executing an ML model. By choosing an appropriate model architecture,
it is possible to keep lookup latencies bound to an acceptible limit.

The core focus of this paper is to outline a design for learned caches
and showcase the design of \name{}, an end-to-end system that leverages learned caches
to speed-up prediction serving without significant trade-off in accuracy.
Below, we highlight the key contributions of this paper -

\noindent (i) We show how to design a learned cache that mimics the function
of a traditional cache lookup. We outline metrics that can be used to evaluate
learned caches and outline design choices that yield desirable values for these metrics
(\secref{sec:learned_cache}).

\noindent (ii) We show that different model architectures for learned caches
induce different trade-offs along the dimensions of cache lookup
latency and cache efficacy. We propose a design that explores this trade-off
space and converges on an optimal choice of model architectures across
the layers of the DNN, while also taking memory and computational constraints
into account (\secref{sec:static-construction}).

\noindent (iii) We design \name{}, an end-to-end system that leverages
learned caches. \name{} takes in a trained DNN model and a validation
dataset and automatically constructs the optimal set of learned caches.
\name{} then deploys these learned caches to be used during inference or
prediction serving (\secref{sec:system-design}).

\noindent (iv) An important property of any cache is the ability to
quickly adapt to changes in the input workload. We show that the learned
cache design is amenable to quick fine-tuning. \name{} has a dedicated
cache updation service that fine-tunes learned caches based on recent
inference queries. In this way, \name{} exploits the temporal locality
inherent in online workloads in order to get early cache hits, which in turn
leads can lead to significant latency gains (\secref{subsec:cache-updation-service}).

\noindent (v)
\name{} allows users to submit inference queries in the form
of a query DAG with a latency SLO, where each node of the DAG corresponds to the
execution of a particular DNN model.
Unlike previous techniques, the use of learned caches
opens up a spectrum of possible latencies, depending on which layer
of the DNN yields a cache hit.
\name{} uses this as an opportunity to dynamically adapt the query execution
plan for a query DAG. \name{} redistributes the additional latency made available
through cache hits to downstream stages of the query DAG, thereby enabling
higher accuracy DNN models to be used in these stages without violating the
latency SLO (\secref{subsec:scheduler}).


==> sections/system-design.tex <==
\section{\name{} System Design}
\label{sec:system-design}

\begin{figure}[t]
  \centering
   \includegraphics[width=0.5\textwidth]{figures/freezer_system_design.pdf}
	\caption{End-to-end system design of \name{}. Awareness of temporal locality is enabled by the cache updation service. Additionally, learned caches open up opportunities for query replanning at the scheduler.}
    \label{fig:system-design}
\end{figure}

We design \name{}, an end-to-end prediction serving system that leverages
learned caches to speed up DNN inference serving (Figure~\ref{fig:system-design}).
Users interact with \name{} in two ways -

\noindent (i) {\em Deployment Phase}: Users can upload a trained
DNN model. The trained model along with a set of constructed
learned caches are then deployed for inference (\secref{subsec:deployment_phase}).

\noindent (ii) {\em Online Phase}: 
Users can issue queries that require executing one or
more DNN models. Queries go through a front-end
query scheduler 
which orchestrates the execution
of the DNN models. A cache adaptation service records samples
of the query inputs and periodically fine-tunes the learned
caches with these samples (\secref{subsec:online_phase}).

\subsection{Deployment Phase}
\label{subsec:deployment_phase}
Users begin DNN deployment by uploading and registering a trained base DNN model.
Additionally, users provide a validation dataset
which can be used by \name{} to develop an initial set of learned caches.

Given the trained DNN and validation dataset, \name{} performs learned cache construction (\secref{sec:static-construction}).
This involves exploring multiple learned cache variants (\secref{subsec:exploration_phase})
and composing an optimal set of learned caches (\secref{subsec:composition_phase}).
The chosen set of learned caches and the base DNN are then stored
in a model repository, which can be any reliable object storage system.
The base DNN and the associated learned caches are then deployed to the inference service.


\subsection{Online Phase}
\label{subsec:online_phase}

Users interact with \name{} by issuing queries.
A query to \name{} consists of the input, a dataflow DAG
corresponding to a sequence of DNN models that need
to be executed as part of the query, and a latency SLO within
which the query need to be executed.
\name{} allows users to specify an array of possible
DNN models that can be used at each node of the
dataflow DAG. This allows users to provide a spectrum
of options ranging from cheaper models with low accuracy
to expensive models with high accuracy.

Queries go through a front-end query scheduler
which is responsible for formulating a query execution plan (QEP),
i.e, a decision of what DNN model needs to be picked for execution
at each node of the dataflow DAG.
\name{} constructs a QEP by splitting the available latency
SLO across each stage of the DAG.
Similar in spirit to ~\cite{grandslam},
\name{} adopts a disaggregated
approach and computes {\em partial latency budgets} 
for each stage of the query DAG (\secref{subsubsec:query_planning}).
Then at every node, the scheduler uses the DNN options specified in the query
to choose a DNN with maximum accuracy
that can execute within the partial latency budget allocated to that node.

Armed with a QEP, the query scheduler orchestrates the
execution of each DNN model by interacting with the inference
service.
The inference service executes the DNN model to arrive
at a prediction. \name{} performs a learned cache lookup after computing layers
for which learned caches are available. The lookup is performed {\em asynchronous}
to the execution of the base DNN model so as to reduce tail
latencies, an aspect we evaluate in \secref{eval_section}.
On getting a cache hit, \name{} terminates the computation of the remaining
layers of the DNN and returns the cached prediction.

The latency of DNN execution depends on which layer of the DNN yields a cache hit.
\name{}s query scheduler exploits this spectrum of latencies
offered by learned caches to replan queries after the execution
of each stage of the DAG (\secref{subsubsec:query_replanning}).

\name{} also sends samples of input queries to the cache
adaption service. This service is responsible for fine-tuning
the learned caches corresponding to a DNN and periodically releasing
new versions of the learned cache that can be used by the
inference service (\secref{subsubsec:cache_adaptation}).

\subsubsection{Computing Partial Latency Budgets}
\label{subsubsec:query_planning}

The query scheduler needs to split the available
latency SLO and compute partial latency budgets for each
node of the DAG.
Borrowing insights from schedulers that support the
execution of a query DAG for prediction serving tasks~\cite{nexus,grandslam},
\name{} currently supports two policies to compute
partial latency budgets -

\noindent {\bf Equal Split. }
This policy splits the latency SLO equally amongst each stage
of the query DAG. If $L$ is the latency SLO for the entire
query and there exist $N$ stages in the query DAG, then
each stage receives a latency budget of $\frac{L}{N}$.

\noindent {\bf Proportional Split. }
This policy splits the latency SLO in proportion to the worst-case
latency of each stage of the query DAG~\cite{grandslam}.
Let us consider a query DAG with $N$ stages and a latency SLO of $L$.
Let us say that each stage $i$ of the query DAG
has a collection of models (with the most expensive model having execution time $C_{i}$) that the query planner needs to choose from.
Each stage receives a latency budget per the below formula -

\begin{scriptsize}
\begin{equation}
	L_{i} = \frac{C_{i}}{\sum_{j=1}^{N}C_{j}}*L
\end{equation}
\end{scriptsize}

\subsubsection{Query Replanning}
\label{subsubsec:query_replanning}

\begin{table}[t]
  \centering
  \begin{scriptsize}
  \begin{tabular}{ c | c | c }
    \hline
          Model & \textbf{Latency} & \textbf{Accuracy} \\
    \hline
          $A_1$ & 25 ms & 90\% \\
    \hline
	  $A_2$ & 50 ms & 95\% \\
    \hline
	  $B_1$ & 20 ms & 90\% \\
    \hline
	  $B_2$ & 30 ms & 95\% \\
    \hline
  \end{tabular}
  \end{scriptsize}
        \caption{Sample model latencies and accuracies for a query}
  \label{tab:query_planning_example}
\end{table}

{\bf A motivating example: }
We use an example to illustrate the opportunity for query replanning
enabled by learned caches.
Let us consider a hypothetical query DAG with two nodes that
need to be executed in sequence.
The first node has two DNN options - $A_1$ and $A_2$.
Similarly, the second has two DNN options - $B_1$ and $B_2$.
Their latencies and accuracies are specified in
Table~\ref{tab:query_planning_example}.
Let us say that the latency SLO is 50 ms.
With an equal split policy, each node would receive
partial latency budgets of 25 ms. With this budget, a query
planner can pick DNN $A_1$ at the first node and $B_1$
at the second node.

Today, DNN executions have static latencies and hence coming
up with such a {\em static} QEP ahead of time is sufficient.
However, learned caches open up a spectrum of latencies
which enables an opportunity to replan the QEP after the execution
of each stage of the DAG.
For instance, if DNN $A_1$ can be executed in 15 ms owing to a
cache hit, then the "saved" latency of 10 ms can be used by the
second node in the DAG, thus giving it a partial latency budget of
35 ms. With this budget, a query planner can choose 
DNN $B_2$ instead of $B_1$ for the second node, thereby resulting
in greater accuracy without violating the latency SLO.

\name{} realizes query replanning by deferring the selection of a particular model at a stage
to when the stage actually needs to execute. Instead, a query scheduler only maintains
partial latency budgets associated with each stage of the dataflow DAG.
When a stage completes execution, the query scheduler computes the {\em saved} latency
by subtracting the observed execution time from the base DNN execution time.
The scheduler then re-distributes this saved latency to downstream stages in accordance with
the policy used to compute partial latency budgets.

\subsubsection{Cache Adaptation Service}
\label{subsubsec:cache_adaptation}

The goal of the cache adaptation service is to {\em fine-tune} learned
caches corresponding to a base DNN so as to exploit the temporal
locality inherently present in online workloads (\secref{}).
Fine-tuning the chosen learned caches allows learned caches to offer better
hit rates, thereby yielding end-to-end latency benefits.

The cache adaptation service records a sample of inputs from the inference
service as shown in Figure~\ref{fig:system-design}.
We maintain a window of samples obtained over time to avoid the effects
of sudden dataset shift and catastrophic forgetting~\cite{}.
Periodically, the cache updation service retrains the predictor
and selector network corresponding to each learned cache
using a mix of data from the window of samples and
the original validation dataset provided by the user.
While picking sampled inputs, we weigh recent sample windows more heavily~\cite{}.
The updated caches are pushed to the model repository. The inference service
periodically pulls new versions of learned caches from the model
repository.

A potential concern in the cache updation service is the storage overhead 
incurred for storing these samples.
Interestingly, our evaluations suggest that sampling just 10\% of inputs
from the inference service is sufficient for exploiting the temporal locality in realistic
workloads (\secref{}), thereby allaying any fears of unrealistic storage requirements.


\begin{comment}
We design \name{}, a system that leverages learned caches to speed up prediction serving.
\todo{Describe high level design here}

\subsection{Initial Upload}
\label{subsec:initial-upload}
Users interact with \name{} by uploading a trained base DNN model and a validation dataset
which will be used by \name{} to generate learned caches.
During this upload, users also required to provide a unique {\em model name} and a
{\em feature name}.
Models that can be used for the same purpose share a common feature name.
For instance, if a user wishes to have two models, say ResNet-18 and ResNet-50
for the same image classification task, then the user can upload both of these
models with the same feature name. \shivaram{the two names seem confusing. Not sure this stuff is
required}

Given the trained DNN and validation dataset, \name{} performs
an offline learned cache construction. This involves going through the exploration phase (\secref{subsec:exploration_phase})
to explore multiple learned cache variants
and then going through the composition phase (\secref{subsec:composition_phase}) to identify the set of optimal learned caches.
The chosen learned cache variants and the base DNN are then stored
in a model repository.
The model repository can be any reliable object storage system
such as Amazon S3~\cite{something}.
The base DNN and the learned caches are then deployed to the inference service (\secref{subsec:inference-service}).


\subsection{Query Model}
\label{subsec:query-model}
\shivaram{We need a running example through this entire section. Draw the DAG you plan to use for
eval and use that?}
Users submit inference queries to \name{} as a dynamic dataflow DAG~\cite{} of DNN model invocations that need to be executed
within a specified latency SLO.
\name{} provides users with two options to specify the choice of the DNN model at each node of the query DAG -

\noindent {\bf Invocation by model name. }
With this option, users specify the exact model name to be executed.

\noindent {\bf Invocation by feature name. }
With this options, users do not specify an exact model name,
but instead specify the type of operation required at each
node through the feature name.
Specifying a feature name gives \name{} the flexibility
to choose any model among the available models with the same feature name.
\name{} chooses a model offering the highest accuracy while ensuring
that the model can execute within the available latency budget.

\subsection{Query Scheduler}
\label{subsec:scheduler}
Users submit inference queries to \name{} using the described query model.
Queries first go through a query scheduler which performs two functions -
(i) Query Routing and (ii) Query Planning.
Each of these are described in separate sections below.

\subsubsection{Query Routing}
\label{subsubsec:query-routing}
\shivaram{Nothing here seems very interesting. Lets get rid of it or just put 1 or 2 lines in the
Query Scheduler sentences above?}
The query scheduler needs to orchestrate the execution of the query DAG.
The query scheduler starts the individual DNN executions and launches
the invocation of downstream dependencies in the query DAG once upstream
dependencies finish execution.

The current prototype of \name{} supports a simple query routing model
that schedules DNN executions in a FIFO manner without batching requests.
\name{} maintains a per-model execution queue of requests for this purpose.
Query routing is a pluggable module and it is possible to incorporate
custom schedulers such as those which use adaptive batching for higher throughput~\cite{clipper}
or batching-aware schedulers for better resource efficiency~\cite{nexus}.
We provide a discussion on the use of batching in \name{} in \secref{}.

\subsubsection{Query Planning}
\label{subsubsec:query_planning}
Given a dataflow DAG representing a query, \name{} needs to come up with
a query execution plan (QEP). In case of invocation by model name,
the choice of the model to be executed is dictated by the model name specified by the user.
However, with invocation by feature name, the query planner needs to pick a model at each
stage of the query DAG such that the end-to-end accuracy of the query is maximized
while not exceeding the latency SLO.

The end-to-end latency of a query is the sum of execution times of DNN executions in each stage
of the query DAG. Similar to \cite{grandslam}, \name{} adopts a disaggregated
approach and calculates partial latency budgets for each stage of the query DAG.
The current prototype of \name{} supports two policies to compute partial latency budgets -
\shivaram{Again use the example to explain how the values will look}

\noindent {\bf Equal Split. }
This policy splits the latency SLO equally amongst each stage
of the query DAG. If $L$ is the latency SLO for the entire
query and there exist $N$ stages in the query DAG, then
each stage receives a latency budget of $\frac{L}{N}$.
\name{} then chooses the model with the highest accuracy
that can execute within the latency budget allocated to the stage.

\noindent {\bf Proportional Split. }
This policy splits the latency SLO in proportion to the worst-case
latencies of each stage of the query DAG~\cite{grandslam}.
Let us consider a query DAG with $N$ stages and a latency SLO of $L$.
Let us say that each stage $S_{i}$ of the query DAG
has a collection of models $C_{i}$ that the query planner needs to choose from.
Each stage receives a latency budget $L_{i}$ per the below formula -

\begin{equation}
	L_{i} = \frac{max(C_{i})}{\sum_{j=1}^{N}max(C_{j})}*L
\end{equation}

Each stage can pick a model with maximum possible accuracy while not exceeding its assigned partial latency budget.
Once a query plan is prepared, the execution of the query DAG proceeds as described in \secref{subsubsec:query-routing}.

\subsubsection{Opportunity for Query Replanning}
Using learned caches at a subset of layers of DNN opens up
a spectrum of possible DNN execution times. This is fundamentally
different from DNN execution today that offer static latencies.
With fixed, known latencies, query planning can be done through
{\em early binding} by picking a fixed execution plan prior to query execution.
\shivaram{Lets not use early binding again -- save that word just for learned cache!}
However, the presence of a latency spectrum in \name{} introduces dynamism and offers an opportunity
for query replanning after the execution of each stage of the query DAG.
Since \name{} provisions the running time of the entire DNN as the execution time of the stage,
a learned cache hit contributes to an increase in the latency budget available to the remaining stages.
\shivaram{Above sentence is very hard to understand. Again connect with the running example}
Query replanning can utilize this additional available latency to select more accurate models,
thereby resulting in greater end-to-end accuracy for the query.

\name{} realizes query replanning by deferring the selection of a model at a stage
to when the stage actually needs to execute. Instead, the only state maintained by the
query scheduler is the latency budget assigned to every stage of the query DAG.
When a stage completes execution, the query scheduler computes the additional latency budget
available by subtracting the observed execution time from the base DNN execution time.
The scheduler then re-distributes this additional latency budget in accordance with
the policy used used to compute partial latency budgets.
\shivaram{Again connect with the running example}


\subsection{Inference Service}
\label{subsec:inference-service}
The inference service is responsible for DNN execution and binding the execution of
models to hardware resources.
The current prototype of \name{} deploys each model and its learned caches on
a single GPU/CPU.
Thus, the memory budget allocated for learned cache composition (\secref{subsec:composition_phase})
is equal to the amount of slack memory available from executing the base DNN.

\name{} overlaps the learned cache computation with the execution of the base DNN.
This ensures that the execution time of any model with learned caches
is bounded by the execution time of the vanilla DNN.
On CPUs, \name{} achieves this by running the base DNN execution and learned cache lookup
in different processes. Each process is pinned to a dedicated set of cores that do not
overlap. This ensures isolation between the computations and guarantees that the execution
time of the base DNN with learned caches does not exceed the execution time of the vanilla
base DNN.
On GPUs, \name{} overlaps computations by using CUDA streams~\cite{}. The base DNN computation
proceeds on the default stream while the learned cache computations are issued on a different
stream.
\shivaram{This can go in implementation as two lines.}
\arjun{CUDA streams does not give isolation guarantees. Need to think about how to talk about this.}


\subsection{Cache Updation Service}
\label{subsec:cache-updation-service}


\subsection{Fault Tolerance}
\label{subsec:fault-tolerance}
\shivaram{I'd suggest removing most of below. You can just say we use a similar deployment model as
Clipper or Nexus in the implementation and thus inherit their fault tolerance properties. The only
interesting bit here is about cache adaptation -- but given space constraints I'd say it can be one
line in the above subsection.}
\name{} assumes the standard fail-stop model in which each of its components
may fail independently at any point of time and whose failure can be detected
using standard liveness detection mechanisms~\cite{zookeeper}.
The base DNN and its associated learned caches are stored in a reliable distributed
storage system~\cite{system1,system2} from where the inference service can load
the latest versions and the cache updation service can write new versions to.
We discuss the failure scenarios of each individual component of \name{} below -

\noindent {\bf Query Scheduler. }
The query scheduler is largely a stateless component and can be restarted upon a failure.
The only state held by the query scheduler is the partial latency budget
for each stage of the query.
\name{} assumes that the entire query execution fails upon the failure of
the query scheduler and hence losing this state upon a crash does not
pose a problem.
For stronger failure resiliance properties, we could replicate the query scheduler
using Apache ZooKeeper~\cite{zookeeper}.

\noindent {\bf Inference Service. }
Like the query scheduler, the inference service is also stateless.
Upon the failure of the inference service, the query scheduler is respondible for 
rescheduling pending DNN execution requests.
Co-locating the learned caches and base DNN models on the same hardware induces
{\em fate-sharing} and circumvents scenarios where the cache is unavailable.

\noindent {\bf Cache Adaptation Service. }
The cache adaptation service holds recorded inference request inputs until
they are used to fine-tune the learned caches.
Failure of the service would result in this data being lost and thereby
limit the ability of \name{} to adapt to temporal locality of workload.
We can adopt two approaches to deal with the failure of this service -

\noindent (i) We can view learned caches as a {\em soft state} entity that
improves performance but whose absence does not affect correctness.
In this model, we can tolerate the failure of cache updation
service without the need to persist any state.
The current prototype of \name{} adopts this model.

\noindent (ii) We can treat learned caches as {\em first-class citizens}
whose timely fine-tuning is crucial to the performance of the system.
In this model, we need to be able to recover the state of recorded
inference input requests upon restart from failure. This can be achieved in
two ways - (a) We can write recorded inference requests to a distributed
file-system~\cite{hdfs} and restore this data upon a restart.
(b) We can replicate the cache updation service using Apache ZooKeeper~\cite{}.
\end{comment}

